Uncovering a Spinor-Vector Duality on a Resolved Orbifold

Spinor-vector dualities have been established in various exact string realisations like orbifold and free fermionic constructions. This paper aims to investigate possibility of having spinor-vector dualities on smooth geometries in the context of the heterotic string. As a concrete working example the resolution of the T4/Z2 orbifold is considered with an additional circle supporting a Wilson line, for which it is known that the underlying orbifold theory exhibits such a duality by switching on/off a generalised discrete torsion phase between the orbifold twist and the Wilson line. Depending on this phase complementary parts of the twisted sector orbifold states are projected out, so that different blowup modes are available to generate the resolutions. As a consequence, not only the spectra of the dual pairs are different, but also the gauge groups are not identical making this duality less apparent on the blowup and thus presumably on smooth geometries in general.

==> FFMTmodel.tex <==
\section{FFMT Model}
\label{sc:FFMTmodel}

This section reviews a simple realization of the spinor--vector duality studied in~\cite{Faraggi:2011aw} on $T^4/Z_2\times T^2$ with a Wilson line on one of the $S^1 \subset T^2$. The second circle was just a spectator in the whole discussion. The model is generated by the basis vectors: 
%
\begin{eqnarray}
v_1&=1=&\{\psi^{1,2}\
\chi^{1,\dots,6}~,y^{1,\dots,6}~, \omega^{1,\dots,6}~|~\bar{y}^{1,\dots,6}~, \bar{\omega}^{1,\dots,6}~;
\bar{\eta}^{1,2,3}~,
\bar{\psi}^{1,\dots,5}~,\bar{\phi}^{1,\dots,8}\}~,\nn\\
v_2&=S=&\{\psi^{1,2}~,\chi^{1,\dots,6}\}~,\nn\\
v_{3}&=z_1=&\{\bar{\psi}^{1,\dots,5}~, {\bar\eta}^{1,2,3}\}~,\nn\\
v_{4}&=z_2=&\{\bar{\phi}^{1,\dots,8}\}~,\nn\\
v_{5}&=b=&\{\chi^{1,\ldots,4}~,y^{1,\ldots,4}~|~\bar{y}^{1,\ldots,4}~;{\bar\eta}^{1,2}\}~,\nn\\ 
v_{6}&=w=&\{y^5~|~\bar{y}^5~;\bar{\eta}^3,\bar{\phi}^8 \}~. 
\label{basis}
\end{eqnarray}
%
 using the two dimensional free fermions in the light--cone gauge:
$\psi^{1,2}$, $\chi^i,y^i, \omega^i, i=1,\dots,6$ (real left--moving fermions)
and
$\bar{y}^i,\bar{\omega}^i, i=1,\dots,6$ (real right--moving fermions),
${\bar\psi}^A, A=1,\dots,5$, $\bar{\eta}^B, B=1,2,3$, $\bar{\phi}^\alpha,
\alpha=1,\ldots,8$ (complex right--moving fermions). The basis vector $S$ is the generator of supersymmetry, $b$ is the $Z_2$ orbifold twist and $w$ defines the Wilson line on the circle in the 5th torus direction. 


The set of basis vectors define the model uniquely up to the free choice of certain generalized GSO phases. In particular, model exhibits a spinor--vector duality induced by the generalized GSO phase: 
%
\begin{equation}
c\big[^b_w\big] = \pm 1~. 
\end{equation}
%
For one choice of the discrete torsion, the zero modes of the untwisted torus in the $\mathcal{N}=2$ twisted sector are attached to the spinorial characters of the GUT group, whereas for the other choice they are attached to the vectorial character. The choices of discrete torsion can be represented as different choices of Wilson line backgrounds~\cite{Faraggi:2011aw}.






